Exploring Prediction Targets in Masked Pre-Training for Speech Foundation Models

Speech foundation models, such as HuBERT and its variants, are pre-trained on large amounts of unlabeled speech data and then used for a range of downstream tasks. These models use a masked prediction objective, where the model learns to predict information about masked input segments from the unmasked context. The choice of prediction targets in this framework impacts their performance on downstream tasks. For instance, models pre-trained with targets that capture prosody learn representations suited for speaker-related tasks, while those pre-trained with targets that capture phonetics learn representations suited for content-related tasks. Moreover, prediction targets can differ in the level of detail they capture. Models pre-trained with targets that encode fine-grained acoustic features perform better on tasks like denoising, while those pre-trained with targets focused on higher-level abstractions are more effective for content-related tasks. Despite the importance of prediction targets, the design choices that affect them have not been thoroughly studied. This work explores the design choices and their impact on downstream task performance. Our results indicate that the commonly used design choices for HuBERT can be suboptimal. We propose approaches to create more informative prediction targets and demonstrate their effectiveness through improvements across various downstream tasks.

==> figures/SeqEn.tex <==
\begin{figure}[tb]
    \centering
    \def\svgwidth{0.7\linewidth}
    \scriptsize
\input{figures_new/fig4_resize.pdf_tex}
    % \includegraphics[width=\linewidth]{figures/SeqEn.pdf}
    \vspace{-5pt}
    \caption{An illustration of the proposed layer multi-target detailed in Section~\ref{ssec:layer_ensemble}.
    H$1$, H$2$, and H$3$ denote different linear heads.
    In sequential multi-target (right), we condition on the ground truth of higher-layer clusters when predicting the lower-layer clusters.
    }
    \label{fig:seq_en}
\end{figure}


==> figures/rvq.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figures/rvq2.pdf}
    \caption{An illustration of the proposed RVQ token prediction approach detailed in Section~\ref{ssec:rvq}.
    We follow the sequential multi-target detailed in Section~\ref{ssec:layer_ensemble} to deal with multiple targets.}
    \label{fig:rvq}
\end{figure}

==> tables_bk/layers-iter2.tex <==
\begin{table*}[tb]
\centering
\caption{Layer to cluster - Iter 2}
\label{tab:layer-iter2}
\begin{tabular}{l|c c c c c}
\toprule
Layers & PER ↓ & ACC (\%) ↑ & PESQ ↑ & STOI ↑ & SI-SDRi ↑ \\
\midrule
Layer 1 & 6.38 & 78.15 & 2.57 & 93.97 & 9.83 \\
Layer 3 & 5.84 & 79.22 & 2.56 & 93.97 & 9.73 \\
Layer 5 & 5.51 & 82.73 & 2.57 & 93.92 & 9.7 \\
Layer 7 & 5.01 & 81.46 & 2.56 & 93.96 & 9.71 \\
Layer 9 & 6.11 & 77.31 & 2.53 & 93.91 & 9.72 \\
Layer 11 & 6.7 & 77.03 & 2.56 & 93.97 & 9.75 \\
\midrule
Ensemble & 6.05 & 79.80 & 2.58 & 94.01 & 9.78 \\
Ensemble (Seq) & 5.63 & 78.16 & 2.57 & 94.04 & 9.88 \\
\bottomrule

\end{tabular}
\end{table*}

==> tables_bk/layers.tex <==
\begin{table*}[tb]
\centering
\caption{Clustering layer v.s. performance. Here we evaluate iteration 3 models trained from clustering different layers of iteration 2. The number of clusters are fixed to be 500.}
\label{tab:clustering_layer}
\begin{tabular}{l|c c c c c}
\toprule
Layers & PER ↓ & ACC (\%) ↑ & PESQ ↑ & STOI ↑ & SI-SDRi ↑ \\
\midrule
Layer 1 & 6.17 & 80.85 & 2.57 & 93.91 & 9.84 \\
Layer 3 & 5.99 & 83.3 & 2.56 & 93.91 & 9.77 \\
Layer 5 & 5.38 & 82.46 & 2.57 & 93.94 & 9.70 \\
Layer 7 & 5.01 & 82.03 & 2.58 & 94.03 & 9.54 \\
Layer 9 & 4.72 & 81.82 & 2.59 & 94.00 & 9.59 \\
Layer 11 & 4.70 & 82.2 & 2.55 & 93.94 & 9.58 \\
\midrule
Ensemble & 4.72 & 84.19 & 2.58 & 94.04 & 9.76 \\
Ensemble (Seq) & 4.49 & 82.37 & 2.57 & 93.88 & 9.79 \\
\bottomrule

\end{tabular}
\end{table*}

==> tables_bk/masking_prob.tex <==
\begin{table*}[tb]
\centering
\caption{Masking Probability}
\label{tab:example}
\begin{tabular}{l|c c c c c}
\toprule
$p$ & PER ↓ & ACC (\%) ↑ & PESQ ↑ & STOI ↑ & SI-SDRi ↑ \\
\midrule
0.2 & 4.97 & 77.37 & 2.56 & 93.95 & 9.21 \\
0.4 & 4.53 & 82.65 & 2.56 & 93.88 & 9.38 \\
0.65 & 4.62 & 82.45 & 2.58 & 93.92 & 9.51 \\
0.8 & 4.72 & 81.82 & 2.56 & 94.00 & 9.59 \\
0.9 & 4.62 & 83.10 & 2.59 & 94.00 & 9.62 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables_bk/n_clusters.tex <==
\begin{table*}[tb]
\centering
\caption{Number of clusters}
\label{tab:n_clusters}
\begin{tabular}{l|c c c c c}
\toprule
\#Clusters & PER ↓ & ACC (\%) ↑ & PESQ ↑ & STOI ↑ & SI-SDRi ↑ \\
\midrule
100 & 4.78 & 83.70 & 2.57 & 93.92 & 9.66 \\
500 & 4.72 & 81.82 & 2.59 & 94.00 & 9.59 \\
2500 & 4.47 & 83.02 & 2.56 & 93.89 & 9.59 \\
5000 & 4.31 & 81.41 & 2.56 & 93.93 & 9.63 \\
10000 & 4.16 & 81.02 & 2.57 & 93.89 & 9.64 \\
25000 & 3.90 & 81.32 & 2.57 & 93.93 & 9.64 \\
50000 & 3.85 & 81.30 & 2.55 & 93.97 & 9.44 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables_bk/n_iters.tex <==
\begin{table*}[tb]
\centering
\caption{Number of iterations v.s. performance. We trained our own iteration 1 model since the official iteration 1 checkpoint is not released.}
\label{tab:n_iter}
\begin{tabular}{l|c c c c c}
\toprule
\#VQ & PR/PER ↓ & SID/ACC(\%) ↑ & SS/SI-SDRi ↑ \\
\midrule
Iter-1 & 8.68 & 72.57 & 2.51 & 93.8 & 9.42 \\
Iter-2* & 5.41 & 81.42 & 2.58 & 93.9 & 9.36 \\
Iter-3 & 4.72 & 81.82 & 2.59 & 94.00 & 9.59 \\
Iter-4 & 4.80 & 81.38 & 2.58 & 93.97 & 9.59 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables_bk/rvq_level.tex <==
\begin{table*}[tb]
\centering
\caption{Number of RVQ-levels}
\label{tab:rvq}
\begin{tabular}{l|c c c c c}
\toprule
RVQ Level & PER ↓ & ACC (\%) ↑ & PESQ ↑ & STOI ↑ & SI-SDRi ↑ \\
\midrule
1 & 4.72 & 81.82 & 2.56 & 94.00 & 9.59 \\
2 & 4.53 & 83.06 & 2.58 & 94.02 & 9.66 \\
3 & 5.80 & 78.74 & 2.57 & 93.96 & 9.84 \\
4 & 7.11 & 76.32 & 2.55 & 93.81 & 9.92 \\
\bottomrule

\end{tabular}
\end{table*}
